Banyan: A Scoped Dataflow Engine for Graph Query Service

Graph query services (GQS) are widely used today to interactively answer graph traversal queries on large-scale graph data. Existing graph query engines focus largely on optimizing the latency of a single query. This ignores significant challenges posed by GQS, including fine-grained control and scheduling during query execution, as well as performance isolation and load balancing in various levels from across user to intra-query. To tackle these control and scheduling challenges, we propose a novel scoped dataflow for modeling graph traversal queries, which explicitly exposes concurrent execution and control of any subquery to the finest granularity. We implemented Banyan, an engine based on the scoped dataflow model for GQS. Banyan focuses on scaling up the performance on a single machine, and provides the ability to easily scale out. Extensive experiments on multiple benchmarks show that Banyan improves performance by up to three orders of magnitude over state-of-the-art graph query engines, while providing performance isolation and load balancing.

==> 1_intro.tex <==

\section{Introduction}\label{sec:introduction}


Graph query service (GQS) is widely used in many Internet applications
ranging from search engines, recommendation systems, to financial risk management.
The global GQS market is estimated to reach $2.9$ billion USD by 2024,
with an annual growth rate of $22.2\%$~\cite{graphdb-annual-growth}.
In these applications, data are represented as large-scale graphs
such as knowledge graphs and social networks, and the explorations on
the data are usually expressed as graph traversal queries.
GQS serves these large-scale graphs for interactive query access,
allowing many users to submit concurrent graph traversal queries
and obtain results in real-time.


Previous graph query engines~\cite{zhao2010graph, yan2016general, sakr2012g, shao2013trinity,
neo4j, janusgraph} mainly focus on optimizing the query latency from the perspective of
computation efficiency, i.e., traversing more vertices/edges in a time unit.
However, we observe that optimizing for computational efficiency \textit{alone}
is not sufficient to achieve short query latency. A multi-tenant GQS needs
to address two key goals to fulfill stringent latency requirements:
(\textbf{O1}) fine-grained control and scheduling,
as well as (\textbf{O2}) performance isolation and load balancing
during the query execution.



\begin{table*}[t]
\footnotesize
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
                                                   			& \textbf{Neo4j} & \textbf{JanusGraph} & \textbf{Timely} & \textbf{GAIA} & \textbf{Banyan}  \\ \hline
\textbf{O1-1: Control on Subquery Traversal}   & \XSolidBrush   & \XSolidBrush        & \XSolidBrush        & \Checkmark    & \Checkmark       \\ \hline
\textbf{O1-2: Subquery-level Scheduling Policy}    			& \XSolidBrush   & query-level only        & \XSolidBrush        & query-level only  & \Checkmark       \\ \hline
\textbf{O2: Subquery-level Isolation} 	& \XSolidBrush   & \XSolidBrush        & \XSolidBrush        & \XSolidBrush  & \Checkmark       \\ \hline
\end{tabular}
\caption{Comparing graph query engines on \textbf{O1} and \textbf{O2}.
TigerGraph~\cite{tigergraph} is not open-sourced and thus not listed.}
\label{table:systems}
\end{table*}


\noindent\textbf{Fine-Grained Control and Scheduling (O1).}
A graph query usually performs many traversals starting
from different source vertices in the graph.
We observe two key techniques that can reduce query latencies,
and in turn boost the system throughput:
(\textbf{O1-1}) concurrently executing these traversals,
and controlling them at a fine granularity;
(\textbf{O1-2}) carefully choosing the traversal strategy.

\\

\begin{example}[A Graph Traversal Query in Gremlin]
\begin{lstlisting}[style=QueryStyle, upquote=false]
g.V(123).repeat(out(`knows'))
    .until(out(`worksAt').is(eq(`XYZ')))
    .or().loops().is(gt(5)))
 .where(in(`tweets').out(`hasTag').is(eq(`#ABC')))
 .limit(20)
\end{lstlisting}
\label{ex:example_query}
\end{example}


Example~\ref{ex:example_query} shows a graph traversal query
intended to find 20 users
who are within the 5-hop neighborhood of
user $123$, work at company `XYZ', and have tweeted with hashtag `\#ABC'.
When executing this query, we need to start a traversal for
every user entering the \textit{where} subquery.
This traversal can be canceled immediately if any tweet of the user
is found to have the desired hashtag, without needing to check all of that user's tweets.
Clearly, canceling this traversal should not affect the traversals for other users.
More importantly, it should not be blocked by other traversals,
e.g., by  someone who tweets a lot but not with hashtag `\#ABC'.
This implies that a GQS needs to support concurrent execution as well as
fine-grained control of subquery traversals (\textbf{O1-1}).

Eagerly checking the hashtags tweeted by one user
requires a DFS scheduling policy for the \textit{where} subquery.
The same scheduling policy holds within one loop iteration in
the \textit{repeat} subquery, as we would like to eagerly check if
a neighbor works at company `XYZ'. However, it would be preferable to use
BFS when scheduling across loop iterations of the \textit{repeat} subquery.
This is because we do not want to blindly explore all neighbors within 5 hops
if 20 candidates can be found in a much smaller neighborhood.
This implies that GQS systems need to support customized traversal policies in subqueries (\textbf{O1-2}).


\noindent\textbf{Performance Isolation and Load Balancing (O2).}
It is challenging to fulfill the stringent latency requirement in a
production environment.
Due to the intrinsic skewness in graph data,
graph traversal queries can vary dramatically in terms of the amount of computation.
Therefore, GQS should be
capable of enforcing performance isolation across queries to guarantee
the latency SLO.
In addition, as illustrated in Example~\ref{ex:example_query},
for better performance, the isolation granularity needs to be as small
as subquery-level traversals.
Existing graph databases~\cite{neo4j, neptune, janusgraph}
map concurrent queries to system threads and rely on the operating system for scheduling.
This mechanism does not expose the internal query complexity
and thus cannot support subquery-level isolation.
The skewness in graph data can lead to dynamic workload skewness at run time,
requiring GQS to provide dynamic load balancing.

% Table 1 shows Banyan's qualitative benefits compared to existing systems.

Table~\ref{table:systems} compares existing graph query engines on their supports for
\textbf{O1} and \textbf{O2}.
Many graph query engines~\cite{neo4jplan, Mellbin, chen2019grasper, gaia, wukong,tigergraph}
use the dataflow model to execute graph traversal queries in languages
such as Cypher~\cite{cypher}, Gremlin~\cite{tinkerpop} and GSQL~\cite{tigergraph}.
Existing dataflow models either a) support only static topologies
(e.g., Timely~\cite{naiad} and GAIA~\cite{gaia}) or b) can only
dynamically spawn tasks at coarse granularity (e.g., CIEL~\cite{murray2011ciel}).
Specifically, Timely and GAIA attach a metadata
(\textit{timestamp} in Timely and \textit{context} in GAIA) in
every message to identify which subquery traversal it belongs to,
but then these systems process messages belonging to different traversals of a
subquery in the same static execution pipeline determined at compile time.
Without physically isolating the execution of traversals inside a subquery,
these systems cannot efficiently support both \textbf{O1} and \textbf{O2}.
Achieving these goals requires flexibly controlling and scheduling
the fine-grained subquery traversals spawned dynamically during query execution.
We expand more in Section~\ref{sec:motivation} to discuss the limitations of
existing dataflow models, and evaluate this issue with experiments in Section~\ref{sec:evaluation}.


In this paper, we propose a novel \textit{scoped dataflow} to model graph traversal queries,
which supports fine-grained control and scheduling during query execution.
The scoped dataflow model introduces a key concept called \textit{scope}.
A scope marks a subgraph in the dataflow, which corresponds to a subquery.
The scope can be dynamically replicated at runtime into physically isolated
scope instances which
correspond to independent traversals of the subquery.
Scope instances can be concurrently executed and independently controlled.
This way, traversals of a subquery can time-share the CPU and be independently canceled
without blocking or affecting each other.
Furthermore, a scope allows users to customize the scheduling policy
between and inside scope instances,
supporting diverse scheduling policies for different parts of a query.

We build the \textit{\gqs{}} engine for a multi-tenant GQS,
based on an efficient distributed implementation of scoped dataflow.
\gqs{} parallelizes a scoped dataflow into a physical plan of operators,
and cooperatively schedules these operators on executors pinned on physical cores.
% \added{Operators process messages in
% a mini-batch granularity and will not occupy an executor for a long time.}
On each executor, \gqs{} dynamically creates and terminates operators
to instantiate and cancel scope instances.
\gqs{} manages operators hierarchically as an operator tree:
operators are scheduled recursively by their parent scope operators.
This hierarchy allows customized scheduling
within each scope, and provides performance isolation
both across queries and within a single query.
\gqs{} partitions the graph into fine-grained \textit{tablets}
and distributes tablets across executors.
To handle workload skewness, \gqs{} dynamically
migrates tablets along with the operators accessing
them between executors for load balancing.
In summary, the contributions of this paper include:




\begin{enumerate}[nosep,leftmargin=*]
  \item We propose the scoped dataflow model, which introduces a novel scope construct to
  a dataflow. The scope explicitly exposes the concurrent execution and control of subgraphs
  in a dataflow to the finest granularity (Section~\ref{sec:scope}).

  \item We build \gqs{}, an engine for GQS based on a distributed
  implementation of the scoped dataflow model. \gqs{} can leverage the many-core parallelism
  in a modern server, and can easily scale out to a distributed cluster (Section~\ref{sec:haf}).

  \item We conduct extensive evaluations of \gqs{} on popular benchmarks.
  The results show that \gqs{} has 1-3 orders of magnitude performance improvement
  over the state-of-the-art graph query engines and provides performance
  isolation and load balancing.
\end{enumerate}


